Tik-Tok: The Utility of Packet Timing in Website Fingerprinting Attacks

A passive local eavesdropper can leverage Website Fingerprinting (WF) to deanonymize the web browsing activity of Tor users. The value of timing information to WF has often been discounted in recent works due to the volatility of low-level timing information. In this paper, we more carefully examine the extent to which packet timing can be used to facilitate WF attacks. We first propose a new set of timing-related features based on burst-level characteristics to further identify more ways that timing patterns could be used by classifiers to identify sites. Then we evaluate the effectiveness of both raw timing and directional timing which is a combination of raw timing and direction in a deep-learning-based WF attack. Our closed-world evaluation shows that directional timing performs best in most of the settings we explored, achieving: (i) 98.4% in undefended Tor traffic; (ii) 93.5% on WTF-PAD traffic, several points higher than when only directional information is used; and (iii) 64.7% against onion sites, 12% higher than using only direction. Further evaluations in the open-world setting show small increases in both precision (+2%) and recall (+6%) with directional-timing on WTF-PAD traffic. To further investigate the value of timing information, we perform an information leakage analysis on our proposed handcrafted features. Our results show that while timing features leak less information than directional features, the information contained in each feature is mutually exclusive to one another and can thus improve the robustness of a classifier.

==> info_leak.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        %
%                                        %
%   EVERYTHING MOVED INTO EXPERIMENTS!   %
%             Do not edit!!!             %
%                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Information Leakage Analysis% of Timing Features
}
\label{infor_leakage}

\begin{figure}[!t]
  \includegraphics[scale=0.70]{figures/timing-clusters.jpg}
  \caption{Feature clustering analysis}
  \label{fig:feat_cluster}
\end{figure}

To gain a better understanding of the value of burst-level timing features, we adopt the WeFDE~\cite{infoleak} technique and perform an information leakage analysis. This technique allows us to estimate the Shannon bits of information that are revealed by particular features. This type of analysis is appealing, as classification accuracy can fail to capture nuance in feature significance. Although the code of WeFDE paper is publicly available, for speed and memory requirements, we re-implemented most of the code ourselves and validated our common results against theirs to ensure consistency.

WeFDE can be organized into two components: an \textit{information leakage analyzer} and a \textit{mutual information analyzer}. The information leakage analyzer uses kernel density estimators to model the distributions of features and ultimately produce an information leakage estimate. The mutual information analyzer is instead responsible for producing metrics describing the amount of shared information, i.e. redundancy, that features have with one another. The mutual information analyzer is used to reduce the number of features for leakage analysis by i) identifying features that share most of their information with other features and are thus redundant, and ii) clustering features that show moderate levels of redundancy. For further details, please refer to the paper by Li et al.~\cite{infoleak}.

For our analysis, we perform two experiments on both our features and timing features previously defined in literature. First, we perform an analysis of the leakage of individual features. This experiment utilizes the WeFDE information leakage analyzer. These results are shown in  Figure~\ref{fig:infoleak}. Second, we use both components of WeFDE to estimate the information leakage of each feature category. These leakages are depicted in Table~\ref{tab:jointleak}. For this experiment, we use the same values for the clustering threshold (0.40) and redundancy threshold (0.90) as used by Li et al.

\input{tables/joint_leakage.tex}

\paragraphX{Results.} In regards to the individual feature leakages, we find that features in the Packets per Second category appear most significant. The highest amount of leakage from any one feature we saw was 2.97 bits. The distribution of leakage values can be summarized as: only 5\% of features leaked more than 1.52 bits of information, 75\% of features leaked less than 1.30 bits, and 50\% of features leak no more than 0.69 bits. In general, the information leakage of most individual timing features is low.

We encountered, however, an interesting finding during our mutual information analysis. When calculating the redundancy value of features pairwise, we found that most features have little shared information, i.e. low redundancy. The mutual information values tended to be substantially below the clustering threshold, and as a result, very few clusters were formed. As such, the majority of timing features do not fall into a cluster and are thus modeled as independent variables during the information leakage analysis. The results of our feature redundancy and clustering analysis is shown in Table~\ref{fig:feat_cluster}. Our redundancy analysis shows that just 40 of the 310 timing features are redundant with at least one other feature. Redundant features most often belonged to the Burst Length, Variance, and IBD-LF categories. In addition, only 32 of the 270 non redundant features could be clustered into five groups. The clusters primarily formed in the previously defined timing feature categories; none of our feature categories formed clusters.

\matt{why are the features in table 4 sorted in this order? should they be most-to-least?}
\nate{sorting is arbitrary. Will change it to sort in descending}
As a result of this clustering behavior, we find that the joint leakage estimates for each category are significantly higher than what the individual leakage results would lead us to anticipate. We find that the category that leaks the most information is Packets per Second at 6.56 bits. The highest leakage for any of our new features is MED at 5.43 bits. Overall, the low redundancy and consequently higher combined leakage of timing features is a good indicator that even minor features add value to the robustness of the classifier.

==> kfp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        %
%                                        %
%   EVERYTHING MOVED INTO EXPERIMENTS!   %
%             Do not edit!!!             %
%                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison of Timing Features with Prior Works}
\label{k_fp_feats_our_feats_compare}
%\nate{added DF feature results and updated the discussion. Allowing the model to train longer increased the acc for both the undef experiments. Unfortunately, the other datasets did not follow the same pattern as the undef. I use this to claim that different classifiers can leverage different features to varying effectiveness. This probably needs to be reviewed}
Table~\ref{tab:cw_k_fp} shows a comparison between the performance of our features and $k$-FP~\cite{hayes2016k} timing features on our datasets. We also examine the features' performance with two classifiers: the $k$-FP Random Forest classifier and the DF model. Our Random Forest (RF) classifier uses the same parameters as the $k$-FP RF classifier, but with adjusted feature sets. The DF model follows the design described in Section~\ref{SecExperiments}.

We see that our features provide less classification value than the packets-per-second and other timing features of $k$-FP. 
%Our features also do not combine well with the $k$-FP features to improve classification accuracy meaningfully. 
When our features are combined with $k$-FP features and used in the RF classifier, we see no noticeable improvement. However, when the combined features are instead used as inputs for the DF model, we see a small accuracy improvement of 2\% for the undefended dataset, indicating that DL is slightly more effective at leveraging the additional information provided by our features. This reinforces the results from Section~\ref{infor_leakage}, which showed that our features capture different, but related timing information.%, however, demonstrates that our features capture different information than their features.

%Interestingly, the effects of the DF model seemed to have both positive and negative effects based on the dataset. Notably, the k-FP features perform worse against the W-T dataset when used in DF, but our features perform 9\% better than when used with the RF classifier. This is not necessarily a surprise as the power of DL lies in its ability to extract hidden features from raw data, which is demonstrated by the performance of our raw-timing attack. Rather, the experiments performed in \textcolor{blue}{Table} ~\ref{tab:cw_k_fp} show that the ability of the classifier to leverage the information contained in a feature can vary based on the classification technique used.



==> tables/5_results_table.tex <==
\begin{table*}[tbp]
%\fontsize{5}{5}
\renewcommand{\arraystretch}{1.25}
  \begin{center}
      \caption{{\bf Closed World:} 10-Fold Cross Validation Performance for each attack in different datasets.}\vskip -0.2cm
    \label{tab:CWresults_k_fold}
    \begin{tabular}{l c c c}
    %\hline
    \textbf{Dataset} & \textbf{Direction}~\cite{Sirinam2018} & \textbf{Raw Timing} & \textbf{Directional Time} \\
    %\begin{tabular}{l c c c c}
    %%\hline
    %\textbf{Dataset} & \textbf{Direction}~\cite{Sirinam2018} & \textbf{Timing Features} & \textbf{Raw Timing} & \textbf{Directional Time} \\
    \hline %\hline
        % before k-fold results
        %Undefended & 98.30\% & 84.32\%  & 96.54\% & \textbf{98.51\%} \\
        %WTF-PAD & 90.70\% & 56.08\% & 84.97\%  & \textbf{93.46\%} \\
        %Walkie-Talkie &  95.20\% & 55.80\% & 74.10\%  & \textbf{95.30\%} \\
        %Onion Sites &  53.30\% & 12.86\% & \textbf{68.90\%}  & 65.50\% \\
        
        % k-Fold results
        %\textbf{Undefended} & $98.37\pm0.09\%$ & 84.32\%  & $96.54\pm0.30\%$ & $98.41\pm0.13\%$ \\
        %\textbf{WTF-PAD} & $90.98\pm0.16\%$ & 56.08\% & $85.93\pm0.62\%$  & $93.46\pm0.65\%$ \\
        %\textbf{Walkie-Talkie} &  $90.54\pm1.09\%$ & $47.48\pm4.60\%$ & $79.59\pm1.93\%$  & $91.23\pm0.63\%$ \\
        %\textbf{Onion Sites} &  $52.51\pm1.31\%$ & $12.86\%$ & $65.88\pm0.95\%$  & $64.65\pm0.86\%$ \\
        % k-Fold results
        \textbf{Undefended} & $98.37\pm0.09\%$  & $96.54\pm0.30\%$ & $98.41\pm0.13\%$ \\
        \textbf{WTF-PAD} & $90.98\pm0.16\%$ & $85.93\pm0.62\%$  & $93.46\pm0.65\%$ \\
        \textbf{Walkie-Talkie} &  $90.54\pm1.09\%$ & $79.59\pm1.93\%$  & $91.23\pm0.63\%$ \\
        \textbf{Onion Sites} &  $52.51\pm1.31\%$ & $65.88\pm0.95\%$  & $64.65\pm0.86\%$ \\
        
    \hline %\hline
    \end{tabular}
  \end{center}
\end{table*}

==> tables/onlyTiming_model.tex <==
\begin{table}[htp!]
\centering
\caption{CNN Model Architecture for Only Timing Experiments.}
\label{my-label}
\begin{tabular}{ll}
\hline
Layer type                & size                      \\ \hline
Convolution + ReLU        & 1 $\times$ 8 $\times$ 32  \\
Convolution + ReLU        & 1 $\times$ 8 $\times$ 64  \\
Convolution + ReLU        & 1 $\times$ 8 $\times$ 128 \\
Fully Connected + ReLU    & 512                       \\
Fully Connected + Softmax & number of classes    \\ \hline
\end{tabular}
\label{cnn_modelarch}
\end{table}

==> tables/rank_timing_feats_table.tex <==
\begin{table*}[tbp]
\fontsize{5}{5}
  \begin{center}
    \caption{Top 20 Features.}
    \label{tab:timeline}
    \begin{tabular}{r c c c c}
       \textbf{Rank} & \textbf{Undefended} &\textbf{WTF-PAD} & \textbf{WT} & \textbf{Onion Sites}\\
      \hline
        \textbf{1} & Interval & IBD-IFF & IBD-LF & IBD-Variance\\
        %\hline
        \textbf{2} & IBD-LF & IBD-Variance & Interval & Interval\\
        %\hline
        \textbf{3} & IBD-Variance & Inter-Intra-Med & IBD-Variance & IBD-LF\\
        %\hline
        \textbf{4} & IBD-FF & IBD-OFF & IBD-Variance & IBD-FF\\
        %\hline
        \textbf{5} & IBD-FF & IBD-LF & Interval & IBD-FF\\
        %\hline
        \textbf{6} & Median & Median & IBD-LF & Inter-Intra-Med\\
        %\hline
        \textbf{7} & IBD-OFF & Interval & IBD-Variance & IBD-FF\\
        %\hline
        \textbf{8} & IBD-IFF & Median & Median & IBD-FF\\
        %\hline
        \textbf{9} & Inter-Intra-Med & Median & Median & Inter-Intra-Med\\
        %\hline
        \textbf{10} & Median & IBD-FF & Inter-Intra-Med & IBD-FF\\
        %\hline
        \textbf{11} & IBD-OFF & IBD-Variance & Interval & Inter-Intra-Med\\
        %\hline
        \textbf{12} & IBD-IFF & Median & IBD-LF & IBD-FF\\
        %\hline
        \textbf{13} & Median & Interval & IBD-Variance & Inter-Intra-Med\\
        %\hline
        \textbf{14} & Inter-Intra-Med & IBD-LF & IBD-Variance & Inter-Intra-Med\\
        %\hline
        \textbf{15} & Median & Median & IBD-Variance & Inter-Intra-Med\\
        %\hline
        \textbf{16} & Median & Median & IBD-FF & IBD-FF\\
        %\hline
        \textbf{17} & Median & Median & Interval & Inter-Intra-Med\\
        %\hline
        \textbf{18} & IBD-Variance & Median & Median & IBD-OFF\\
        %\hline
        \textbf{19} & IBD-FF & IBD-LF & IBD-LF & Inter-Intra-Med\\
        %\hline
        \textbf{20} & IBD-LF & Interval & Median & IBD-FF\\
       \hline %\hline
    \end{tabular}
  \end{center}
\end{table*}

==> tables/wtfpad_leakage.tex <==
\begin{table}[tbp]
%\fontsize{5}{5}
\renewcommand{\arraystretch}{1.25}
  \begin{center}
      \caption{Information leakage for the WTF-PAD dataset (our features*).}\vskip -0.2cm
    \label{tab:wtfpadleakage}
    \begin{tabular}{l c}
    %\hline
    \textbf{Feature Category} & \textbf{Leakage (bits)} \\
    \hline %\hline
        \textbf{Pkt. per Second} & 6.56 \\
        \textbf{MED*} & 4.75 \\
        \textbf{Time Statistics} & 4.68 \\
        \textbf{IBD-IFF*} & 3.71 \\
        \textbf{IBD-OFF*} & 3.68 \\
        \textbf{IBD-FF*} & 3.51 \\
        \textbf{IMD*} & 3.45 \\
        \textbf{Variance*} & 1.69 \\
        \textbf{Burst Length*} & 1.66 \\
        \textbf{IBD-LF*} & 1.66 \\

    \hline %\hline
    \end{tabular}\vskip -0.5cm
  \end{center}
\end{table}

% WTF-PAD Leakage
%   PKT_PER_SEC  : 6.56
%   MEDIANS      : 4.75
%   PKT_TIME     : 4.68
%   IBDIFF       : 3.71
%   IBDOF        : 3.68
%   IBDFF        : 3.51
%   IMD          : 3.45
%   VARIANCE     : 1.69
%   IBDLF        : 1.66
%   BURST LENGTH : 1.66
